What is essential is visible to the eye: Saliency in primary school ranking and its effect on academic achievements

We propose a new strategy to identify the impact of class rank, exploiting a "visible" primary school rank from teachers' exam grades, and an "invisible" rank from unreported standardized test scores. Leveraging a unique panel dataset on Italian students, we show that the visible rank has a substantial impact on students' perceptions, which affects subsequent academic performance. However, the effect of being surrounded by higher-SES or higher-achieving peers remains positive even accounting for the decrease in rank. Higher-ranked students self-select into high schools with higher average student achievements. Finally, exploiting an extensive survey, we identify psychological mechanisms channeling the rank effect.

==> tables/desc_stat_cohort/desc_stat_cohort_ties.tex <==

\begin{table}[H] \centering \begin{threeparttable}[b]  \footnotesize
\caption{Distribution of Rank Ties} \label{tab:cohort_ties_distrib}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{lcc}
\toprule
Rank based on ... & Mean & Median \\ 
\midrule
Class Grade &    4.5  & 4  \\
Standardized Test Grades &   0.21  &   0 \\
\bottomrule
\end{tabular}
\begin{tablenotes} \setstretch{1}
\textbf{Note:} This Table reports the mean and median of the number of rank ties for each student in our sample according to the type of grade.
\end{tablenotes}
\end{threeparttable}
 \end{table}

==> tables/mechanisms/desc_stat_cohort2018_students_chara_restricted.tex <==

\begin{table}[H] \centering \begin{threeparttable}[b]  \footnotesize
\caption{Students Characteristics} \label{tab:cohort2018_students_chara_restricted}
\renewcommand{\arraystretch}{0.9}
\vspace{-.5cm}
\begin{tabular}{lM{8em}M{8em}M{12em}}
\toprule
& Mean & Std. Dev. & Obs. \\ 
 \midrule 
\multicolumn{4}{l}{\textbf{2018 Cohort: Restricted Sample}} \\
\hspace{0.4cm} Socio-Economic Status &    0.10  &    0.96 &   173,932 \\
\hspace{0.4cm} \% of Women &    0.52  & 0.50 &     173,932 \\
\hspace{0.4cm} \% of Immigrants &    0.08  &    0.27 &   173,932 \\
\multicolumn{4}{l}{\textbf{2018 Cohort: All Sample}} \\
\hspace{0.4cm} SES &    0.01  &    1.00 &     457,146 \\
\hspace{0.4cm} \% of Women &    0.49  &    0.50 &       496,331 \\
\hspace{0.4cm} \% of Immigrants &    0.20  &    0.40 &  496,331 \\
\bottomrule
\end{tabular}
\begin{tablenotes} 
\textbf{Note:} \setstretch{1} This Table compares the selected sample for the mechanism analysis of Section \ref{subsec:mecha_motivation} to the baseline sample of students observed in High school (Grade 10) in 2018. See Section \ref{subsec:mecha_motivation} for details. 
\end{tablenotes}
\end{threeparttable}
 \end{table}

==> tables/rank_vs_class_effects/comparison_rank_vs_class_effect.tex <==
 \begin{table}[H]\centering
\begin{threeparttable}[b]
\caption{Rank Effect vs. Class Effect}\label{tab:rankeffect_vs_classeffect}
\footnotesize
\label{table}
\begin{tabular}{lM{17em}M{17em}}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c}{Performance in ..} \\
 & Middle School (Grade 8) & High School (Grade 10)  \\
\midrule
 Class Rank & 2.09 & 2.18 \\
 Class Quality & 12.31 & 12.64 \\
\midrule
Ratio & 17.0\% & 17.2\% \\
\bottomrule 
\end{tabular} 
\begin{tablenotes}
\setstretch{1} \textbf{Note:} This Table reports the effect on subsequent academic achievements of one standard deviation increase in the Primary school class rank and in the Primary school class quality. These effects are computed from Equation \ref{eq:main_specification}, with the class quality effect being estimated from class-by-subject fixed effects. See Section \ref{sec:rankvsclass} for details. 
\end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/robcheck/robcheck_coverage_random_cohort.tex <==
\begin{table}[H]\centering
\begin{threeparttable}[b]
\caption{Monte Carlo Simulations - Missing Students}
\small
\label{tab:robcheck_coveragerandom_bs}
\vspace*{0.4cm}
\begin{tabular}{l M{6.5em} M{6.5em}}
\toprule
& Grade 8 & Grade 10 \\
\midrule
$\hat{\beta}$	&	$9.04$	&	$7.81$	\\
IQR	&	[8.83-9.23]	&	[7.61-8.00] \\
\bottomrule 
\end{tabular} 
\begin{tablenotes}\textbf{Note:} This table shows the result of 200 Monte Carlo simulations estimating Equation \ref{eq:main_specification} after randomly allocating class scores to missing students and recomputing ranks accordingly. IQR reports the 25th and 75th percentiles. 
\end{tablenotes}
\end{threeparttable}
\end{table}


==> tables/robcheck/temporal_mismatch.tex <==
\begin{table}[H]%
\caption{Temporal Mismatch}%
 \label{temporal_mismatch} %
 \scriptsize \centering %
 \begin{threeparttable} %
\begin{tabular}{lM{6.8em}M{6.8em}}%
\vspace{0mm}\\%
 \toprule%
 \toprule
 & \multicolumn{2}{c}{Performance in Grade 8}
&(1)&(2)\\%
\midrule%
Visible Rank&7.331***&7.224***\\%
&(0.983)&(1.030)\\%
Grade 5 Undisclosed Rank&0.816&0.787\\%
&(0.525)&(0.547)\\%
Grade 2 Undisclosed Rank&&{-}0.461\\%
&&(0.566)\\%

& \\
Observations&434,458&434,458\\%
\bottomrule%
\end{tabular}%
\begin{tablenotes} \regfootnotesrobcheckcontrol \end{tablenotes}%
\end{threeparttable}%
\end{table}
